Learning Priors for Adversarial Autoencoders

Most deep latent factor models choose simple priors for simplicity, tractability or not knowing what prior to use. Recent studies show that the choice of the prior may have a profound effect on the expressiveness of the model,especially when its generative network has limited capacity. In this paper, we propose to learn a proper prior from data for adversarial autoencoders(AAEs). We introduce the notion of code generators to transform manually selected simple priors into ones that can better characterize the data distribution. Experimental results show that the proposed model can generate better image quality and learn better disentangled representations than AAEs in both supervised and unsupervised settings. Lastly, we present its ability to do cross-domain translation in a text-to-image synthesis task.

==> reference.tex <==
\begin{thebibliography}{1}

\bibitem{1}
A. B. L. Larsen, S. K. Sønderby, H. Larochelle, and O. Winther, “Autoencoding beyond pixels using a learned similarity metric,” \emph{arXiv:1512.09300 [cs, stat]}, Dec. 2015.

\bibitem{2}
N. Dilokthanakul et al., “Deep Unsupervised Clustering with Gaussian Mixture Variational Autoencoders,” \emph{arXiv:1611.02648 [cs, stat]}, Nov. 2016.


\bibitem{3}
A. Makhzani, J. Shlens, N. Jaitly, I. Goodfellow, and B. Frey, “Adversarial Autoencoders,” \emph{arXiv:1511.05644 [cs]}, Nov. 2015.

\bibitem{4}
J. Wu, C. Zhang, T. Xue, W. T. Freeman, and J. B. Tenenbaum, “Learning a Probabilistic Latent Space of Object Shapes via 3D Generative-Adversarial Modeling,” \emph{arXiv:1610.07584 [cs]}, Oct. 2016.


\bibitem{5}
D. P. Kingma and M. Welling, “Auto-Encoding Variational Bayes,” \emph{arXiv:1312.6114 [cs, stat]}, Dec. 2013.


\bibitem{6}
Y.~Yorozu, M.~Hirano, K.~Oka, and Y.~Tagawa, ``Electron spectroscopy
studies on magneto-optical media and plastic substrate interface,''
\emph{APSIPA Transl. J. Magn. Japan,} vol. 2, pp. 740-741, August 1987
[\emph{Digests 9$^{\rm th}$ Annual Conf. Magnetics Japan,} p. 301,
1982].

\bibitem{7}
M.~Young, \emph{The Technical Writer's Handbook.} Mill Valley, CA:
University Science, 1989.

\end{thebibliography}
